Controllable Text Generation with Language Constraints

We consider the task of text generation in language models with constraints specified in natural language. To this end, we first create a challenging benchmark Cognac that provides as input to the model a topic with example text, along with a constraint on text to be avoided. Unlike prior work, our benchmark contains knowledge-intensive constraints sourced from databases like Wordnet and Wikidata, which allows for straightforward evaluation while striking a balance between broad attribute-level and narrow lexical-level controls. We find that even state-of-the-art language models like GPT-3 fail often on this task, and propose a solution to leverage a language model's own internal knowledge to guide generation. Our method, called CognacGen, first queries the language model to generate guidance terms for a specified topic or constraint, and uses the guidance to modify the model's token generation probabilities. We propose three forms of guidance (binary verifier, top-k tokens, textual example), and employ prefix-tuning approaches to distill the guidance to tackle diverse natural language constraints. Through extensive empirical evaluations, we demonstrate that CognacGen can successfully generalize to unseen instructions and outperform competitive baselines in generating constraint conforming text.

==> 4_data.tex <==

\section{Datasets}\label{sec:data}


\subsection{Constraint Dataset Construction}
Exsiting benchmarks for controlling generation mainly focus on reducing toxicity, transferring style, mapping tabular data to text, or steering the model to generate text given high-level sentiment or topical control code. We focus on assessing the model's ability to stay on topic and avoid violating constraint, which requires leveraging its own knowledge and using it appropriately during generation.
To this end, we construct two datasets: 1) a hierarchical constraint dataset based on WordNet and 2) a constraint dataset based on Wikidata.

\kn{Might be worth adding 1 example from each dataset in a table, along with the sampled latent variables like $\bar{t}$, $\bar{c}$, etc. to make our collection process easier to understand.}

\paragraph{WordNet.}
We use WordNet \cite{} and its hypernymy relation to construct a hierarchical constraint dataset. We select $5$ root nodes ``animal'', ``vehicle'', ``art'', ``food'', and ``sport'' from which the hierarchical structure is constructed. The leaf nodes are instances of their ancestors and are used as the topic and constraint checker.
Concretely, when evaluating the generated text $x$ against a constraint entity $\constword$ using the WordNet constraint checker: $\ccheck^{\text{wordnet}} (x, \constword) = \mathbbm{1}[ x \cap \leafs(\constword)$ ].
For each leaf node and its predecessor node (e.g., $\texttt{leaf}: \text{``Labrador''}, \texttt{predecessor}: \text{``dog''}$, we scrape from Wikipedia the corresponding sentences in the first paragraph that contains it. 
We sample two nodes within the same sub-tree from the WordNet hierarchy, where the higher-level node is the topic, and the lower-level node is the constraint. Finally, we sample $3$ leaf nodes from below the topic node and use them as demonstrations ($\lvert \xdemos \rvert = 3$).
Each example is constructed by: 1) sample a node as the topic, 2) sample $\lvert \xdemos \rvert = 3$ nodes under the topic node, and 3) generate continuation from GPT2-XL and use the generated node as the constraint.
We collect a dataset of train/develop/test split of \todo{XX} examples.


\paragraph{Wikidata.}
We use Wikidata \cite{} to construct the constraint dataset. Each entity in Wikidata is characterized by a property and its value ($\texttt{property}: \text{``occupation''}$, $\texttt{value}: \text{``politician''}$). We use \todo{XX} properties from Wikidata (\S\ref{appx:appendix}).
We scrape from Wikipedia the corresponding first sentence of each entity.
Each example is constructed by: 1) first sample a property and a value as the topic, 2) sample $\lvert \xdemos \rvert = 3$ entities from the property-value set, and 3) generate continuation from GPT2-XL and use the generated entity as the constraint.
We collect a dataset of train/develop/test split of \todo{XX} examples.


\paragraph{Diverse instruction templates.}
Our goal is to assess the model's ability to understand instructions that are diversely verbalized. For example, the templates include instructions where the order of the topic and constraint vary and the lexical context differ (see \S\ref{appx:appendix} for examples).
We collect \todo{XX} templates to reflect he diverse nature of the instructions.


\subsection{Metrics}

We evaluate on two axies: 1) the model's ability to stay on topic and avoid violating constraint, and 2) maintaining fluency.

\paragraph{Instruction Conformance (IC).}
The primary metric we use is whether the generation $x$ conforms to the constraint $c$ while staying on topic $t$:
\begin{align}
    \text{IC} = \sum_{x \in \mathcal{D}} \frac{\mathbbm{1} [ \tcheck(x, \topicword) = 1 ] \cdot \mathbbm{1} [ \ccheck(x, \constword) = 1 ]}{\lvert \mathcal{D} \rvert}.
\end{align}
A higher IC indicates that the model is able to generate text that conforms to the constraint while staying on topic.
We also report the on-topic score $\sum_{x \in \mathcal{D}} \frac{\mathbbm{1} [ \tcheck(x, \topicword) = 1 ] }{\lvert \mathcal{D} \rvert}$ (higher is better) and the constraint violation score $\sum_{x \in \mathcal{D}} \frac{\mathbbm{1} [ \ccheck(x, \constword) = 1 ] }{\lvert \mathcal{D} \rvert}$ (lower is better).

\paragraph{Copy-BLEU.}
We report the extent to which the generation undesirably copies from the demonstrations. The copying BLEU is calculated by taking the maximum BLEU score between the generated text and the $\lvert \xdemos \rvert$ demonstrations. The lower the copying BLEU, the less the generation copies from the demonstrations, hence more desirable.

\paragraph{Repetition.}
We report the ratio of repetition (lower is better) in the generated text (\textbf{seq-rep-n}) proposed in \citet {welleck2020unlikelihood}. 

\paragraph{Perplexity (PPL).}
We report the perplexity (lower is better) of the generated text. Perplexity is calculated with respect to GPT2-XL in the generated sentence.

